Fast Conditional Network Compression Using Bayesian HyperNetworks

We introduce a conditional compression problem and propose a fast framework for tackling it. The problem is how to quickly compress a pretrained large neural network into optimal smaller networks given target contexts, e.g. a context involving only a subset of classes or a context where only limited compute resource is available. To solve this, we propose an efficient Bayesian framework to compress a given large network into much smaller size tailored to meet each contextual requirement. We employ a hypernetwork to parameterize the posterior distribution of weights given conditional inputs and minimize a variational objective of this Bayesian neural network. To further reduce the network sizes, we propose a new input-output group sparsity factorization of weights to encourage more sparseness in the generated weights. Our methods can quickly generate compressed networks with significantly smaller sizes than baseline methods.

==> method-bac.tex <==
While the Bayesian compression framework of \cite{louizos2017bayesian},
explained in Section~\ref{subsec:Bayesian-compression}, provides
a principled way for unconditional compression, it is not clear how
to tune it to work in practical contexts with specific resource constraints.
Thus we formulate a \emph{new problem of conditional compression},
where we infer the network sparsity and bit precision \emph{on-the-fly}
conditioned on a specified context.

The compression context can be ideally arbitrary. In this work, we
focus on three general types of conditioning context: (a) the subset
of input features, (b) the subset of output classes, and (c) the expected
model size. The input feature condition means that the feature or
data distribution is limited to some subspace or input region, for
example a subset of image channels or a subset of vocabulary. The
output classes condition means that the classification output is limited
to some sub-classes. The model size constraint reflects resource specification
such as memory footprint, and this translates to reaching an equivalent
compression rate for a given pre-trained network.

We then propose a new Bayesian framework to solve the problem, employing
neural hypernetworks \cite{ha2016hypernetworks} to generate the distribution
of compressed networks given the conditions. We term this new framework
BHC, which stands for \textbf{B}ayesian \textbf{H}ypernetwork \textbf{C}ompression.


\subsection{Conditional Bayesian hypernetworks}
\begin{center}
\emph{}
\begin{figure}
\begin{centering}
\emph{\includegraphics[viewport=0bp 0bp 280bp 170bp,clip,height=4cm]{fig/graphical-model-hypernet}}
\par\end{centering}
\emph{\caption{The graphical model of our conditional compression framework. $W_{0}$
is the pretrained network weights trained on the dataset $\protect\Dcal_{0}=\{(x_{0}^{n},y_{0}^{n})\}_{n=1}^{N}$.
$W_{0}$ is used to initialize the hypernetwork $\gamma$ to generate
the initial means and variances of weights $W_{t}$. For each context
$t$, the hypernetwork $\gamma$ generates a compressed $W_{t}$ conditioned
on $z_{t}$ (and $c_{t}$ implicitly). Then it is used for the classification
context on \emph{$\protect\Dcal_{t}=\{(x_{t}^{m},y_{t}^{m})\}_{m=1}^{M}$}.
When$W_{0}$ is absent, the framework can also be trained from scratch
to generate $W_{t}$ for each context $t$. \label{fig:Conditional-compression-framework}}
}
\end{figure}
\par\end{center}

Let $W_{0}$ be the pretrained network weights trained on the dataset
$\Dcal_{0}=\{(x_{0}^{n},y_{0}^{n})\}_{n=1}^{N}$. We aim to quickly
generate a compressed network $W_{t}$ from $W_{0}$ in some context
$t$ with a constraint on the data domain or the compute resource,
denoted by the condition $c_{t}$, i.e., $W_{t}=f_{\gamma}(c_{t},W_{0})$
for some hypernetwork $f_{\gamma}$ parameterized by $\gamma$. In
theory we can train $f$ by running external compression algorithms
with varying conditions to collect training data, but this is extremely
expensive to cover the large condition space.

Inspired by the Bayesian compression framework of \cite{louizos2017bayesian}
(see Section~\ref{subsec:Bayesian-compression}), we introduce a
new efficient Bayesian framework, in that $W_{t}$ is probabilistically
generated by the hypernetwork at training time and the posterior of
$W_{t}$ from the condition $c_{t}$ is estimated at inference time.
Fig.~\ref{fig:Conditional-compression-framework} shows the graphical
model of the proposed method.

In this framework, we are given a set of $T$ classification scenarios
(or contexts) $\Dcal=\{(\Dcal_{t},c_{t})\}_{t=1}^{T}$, each containing
classification data $\Dcal_{t}=\{(x_{t}^{m},y_{t}^{m})\}_{m=1}^{M}$
and constraint $c_{t}$. Marginalizing over all condition $c_{t}$'s
then gives the posterior distribution of $W_{t}$, $q(W)=\int q(W_{t}|c_{t})p(c_{t})dc_{t}$,
which is a continuous mixture distribution with mixing density $p(c_{t})$.
The compression is done by minimizing the KL distance from a normal-Jeffreys
group sparsity prior to the weight posterior \cite{louizos2017bayesian}.
At test time, the hypernetwork generates a mask and the posterior
mean of $W_{t}$ to produce a compressed deterministic network for
classification on $\Dcal_{t}$.

We solve this problem by modeling the joint distribution between the
parameter $W$, the dropout mask $z$, and the condition $c$. First,
we assume each mask is a latent variable associated with a given condition,
and their joint distribution factors as $p(c,z)=p(c|z)p(z)$. We aims
at learning an optimal variational posterior distribution $q_{\beta}(z|c_{t})$
given this condition such that the weight $W$ is sparse and still
performs well on the (conditioned) dataset $\Dcal$. That is we maximize
the variational objective:
\begin{align}
\max_{\beta}~ & \mathbb{E}_{z\sim q_{\beta}(z|c)}\left[\log p(\Dcal\mid W,z)+\lambda_{c}\log p(c\mid z)\right]\nonumber \\
 & -\lambda_{KL}\left(\Ebb_{q_{\phi}(z)}\left[KL\left(q_{\phi}(W|z)\|p(W|z)\right)\right]+\KLD\left(q_{\phi}(z|c)\|p(z)\right)\right)\label{eq:conditional-objective}
\end{align}



\subsection{Compression contexts}

For the sparsity condition that directly limits the network capacity,
we observe that varying the cutoff threshold on the logarithm of dropout
rates can produce networks with varying compression rate. The normal-Jeffreys
prior give rise to a continuum of the dropout domain in the scale
posterior which supports compression at various rate. Whereas the
horseshoe prior tends to separate the compression rates into two isolated
clusters. However, even for the normal-Jeffreys prior, we observe
that the accuracy will degrade significantly if the required compression
rate is significantly higher than its attained compression rate at
convergence. Therefore we proposed an additional level of compression
in addition to the group sparsity induced by the normal-Jeffreys prior
and use the hypernetwork to select the level of compression given
the required sparsity condition.

\subsection{Group sparsity and input-output group sparsity reparameterization}

In \cite{louizos2017bayesian}, the author proposed coupling the scales
of weights belonging to the same input neuron by sharing the scale
variable $z$ in the joint prior as well as in the joint posterior,
\begin{align*}
p(W,z) & \propto\prod_{i}^{A}\frac{1}{|z|}\prod_{i,j}^{A,B}\Ncal(w_{ij}|0,z_{i}^{2})\\
q_{\phi}(W,z) & =\prod_{i}^{A}\Ncal(z_{i}|\mu_{z_{i}},\sigma_{z_{i}}^{2})\prod_{i,j}^{A,B}\Ncal(w_{ij}|z_{i}\mu_{ij},z_{i}^{2}\sigma_{ij}^{2})
\end{align*}

This group sparsity distribution $p(z)$ is applied to the input of
a layer with weight $W$. For deep networks with multiple layers $\{W_{l}\}_{1}^{L}$,
we observe that the input sparsity $z^{l}$ of a layer $W_{l}$ should
directly affect the input sparsity of the next layers. Therefore we
introduce and additional scale variable $s$ for the output and propose
to use a joint input-output group sparsity as follow,

\begin{align*}
p(W,z,s) & \propto\prod_{i}^{A}\frac{1}{|z_{i}|}\prod_{j}^{B}\frac{1}{|s_{j}|}\prod_{i,j}^{A,B}\Ncal(w_{ij}|0,z_{i}^{2}s_{j}^{2})\\
q_{\phi}(W,z,s) & =\prod_{i}^{A}\Ncal(z_{i}|\mu_{z_{i}},\sigma_{z_{i}}^{2})\prod_{j}^{B}\Ncal(s_{j}|\mu_{s_{j}},\sigma_{s_{j}}^{2})\prod_{i,j}^{A,B}\Ncal(w_{ij}|z_{i}s_{j}\mu_{ij},z_{i}^{2}s_{j}^{2}\sigma_{ij}^{2})
\end{align*}

Note that this method applies to activation functions which have a
zero fixed point, such as tanh, RELU, and ELU families, in order for
the output group sparsity to carry on to the next layer input\footnote{We assume the bias, if exist, can be included into the weight matrix
and the input is augmented by a constant one.}. This creates a ``pairwise'' sparsity coupling one layer and the
next layer since the output feature map of one layer will be the input
to the next layer, where its sparsity pattern will be taken into account.
This coupling of the input-output sparsity directly help increase
the sparsity level of the network, thus can be used to achieve higher
compression level. In the forward step the weights $W$ is sampled
conditioned on the sparsity of both the input, via $z$, and the output,
via $s$. In the backward step, the gradient of $W$ is passed directly
to update the input and output scales in pair.

The variational lower bound under this new prior and posterior is:

\begin{align}
\Lcal(\phi) & =\Ebb_{q_{\phi}(z,s)q_{\phi}(W|z,s)}[\log p(\Dcal|W)]+\nonumber \\
 & \hspace{5mm}-\lambda_{KL}\left(\Ebb_{q_{\phi}(z,s)}[KL(q_{\phi}(W|z,s)\|p(W|z,s))]+KL(q_{\phi}(z,s)\|p(z,s))\right)\label{eq:conditional-objective-detail}
\end{align}
where $\lambda_{KL}$ is the weighting factor to control the level
of compression, which we will utilize in the experiments for different
level of compression requirements. The negative KL divergence from
the joint normal-Jeffreys scale prior to the joint Gaussian posterior
in this new parameterization is as follow:

\begin{align*}
-KL(q_{\phi}(z,s)\|p(z,s))\approx & \sum_{i}^{A}\left(k_{1}\sigma(k_{2}+k_{3}\log\alpha_{i})-0.5m(-\log\alpha_{i})-k_{1}\right)\\
 & +\sum_{j}^{B}\left(k_{1}\sigma(k_{2}+k_{3}\log\beta_{j})-0.5m(-\log\beta_{j})-k_{1}\right),
\end{align*}
where $\sigma(.)$, $m(.)$ are the sigmoid and softplus functions
and $k_{1}=0.63576$, $k_{2}=1.87320$, $k_{3}=1.48695$.

At test time, we use the posterior mean of $W$and apply the masks
$M=m_{z}m_{s}^{T}$ to output the deterministic weight matrix,
\begin{equation}
\hat{W}=M\odot\Ebb_{q_{\phi}(z,s)q_{\phi}(\tilde{W})}\left[\text{diag}(z)\tilde{W}\text{diag}(s)\right]=\text{diag}(m_{z}\odot\mu_{z})M_{W}\text{diag}(m_{s}\odot\mu_{s})\label{eq:mask}
\end{equation}
 where the mask $M=m_{z}m_{s}^{T}$ is the binary mask matrix determined
using the input mask $m_{z}$ and output mask $m_{s}$. We use the
following variational posterior marginal variance to determine the
bit precision of the weights:

\[
\Vbb(w_{ij})=\Vbb(z_{i}\tilde{w}_{ij}s_{j})=(\sigma_{z}^{2}+\mu_{z}^{2})(\sigma_{ij}^{2}+\mu_{ij}^{2})(\sigma_{s}^{2}+\mu_{s}^{2})-\mu_{z}^{2}\mu_{ij}^{2}\mu_{s}^{2}
\]


\subsection{Training methods}

We train the Bayesian compression models then quickly adapt to each
condition using our framework. Therefore, when there is no condition,
our method generates the compressed network which matches the performance
of existing Bayesian compression networks. However when there are
extra context information, we can input into our hypernetwork to generate
a tailored, highly compressed network for that specific context. We
demonstrate various contextual scenarios, including domain context,
subclass context, and compute resource context in the next section.

\begin{algorithm}
\begin{algor}[1]
\item [{Require:}] input $H$, hypernetwork $f_{\phi}$, condition $c\sim p(c)$
\item [{{*}}] $M_{w},\Sigma_{w},\mu_{z},\sigma_{z},\mu_{s},\sigma_{s}=f_{\phi}(c)$
\item [{{*}}] $E_{z}\sim\Ncal(0,1)$
\item [{{*}}] $Z=\mu_{z}+\sigma_{z}\odot E_{z}$
\item [{{*}}] $\hat{H}=H\odot Z$
\item [{{*}}] $E_{s}\sim\Ncal(0,1)$
\item [{{*}}] $S=\mu_{s}+\sigma_{s}\odot E_{s}$
\item [{{*}}] $M_{h}=S\odot M_{w}\hat{H}$
\item [{{*}}] $V_{h}=S^{2}\odot\Sigma_{w}\hat{H}^{2}$
\item [{{*}}] $E\sim\Ncal(0,1)$
\item [{{*}}] return $M_{h}+\sqrt{V_{h}}\odot E$
\end{algor}
\caption{Feedforward pass algorithm of BHC for fully connected layer. \label{alg:fc-algorithms.}}
\end{algorithm}

\begin{algorithm}
\begin{algor}[1]
\item [{Require:}] input $H$, hypernetwork $f_{\phi}$, condition $c\sim p(c)$
\item [{{*}}] $M_{w},\Sigma_{w},\mu_{z},\sigma_{z},\mu_{s},\sigma_{s}=f_{\phi}(c)$
\item [{{*}}] $E_{z}\sim\Ncal(0,1)$
\item [{{*}}] $Z=\mu_{z}+\sigma_{z}\odot E_{z}$
\item [{{*}}] $\hat{H}=H\odot Z$
\item [{{*}}] $E_{s}\sim\Ncal(0,1)$
\item [{{*}}] $S=\mu_{s}+\sigma_{s}\odot E_{s}$
\item [{{*}}] $S=\text{reshape}(S,[1,1,F,N])$
\item [{{*}}] $M_{h}=S\odot M_{w}*\hat{H}$
\item [{{*}}] $V_{h}=S^{2}\odot\Sigma_{w}*\hat{H}^{2}$
\item [{{*}}] $E\sim\Ncal(0,1)$
\item [{{*}}] return $M_{h}+\sqrt{V_{h}}\odot E$
\end{algor}
\caption{Feedforward pass algorithm of BHC for convolution layer. \label{alg:cnn-algorithms.}}
\end{algorithm}

Algorithms~\ref{alg:fc-algorithms.} and \ref{alg:cnn-algorithms.}
show the forward pass of BHC networks for fully connected and convolution
layers respectively. In each algorithm, $M_{w}$, $\Sigma_{w}$ are
the generated means and variances of each layers, $\mu_{z}$, $\sigma_{z}$
are the means and variances of the input group scale variables, $\mu_{s}$,
$\sigma_{s}$ are the means and variances of the input group scale
variables, $H$ is the input to the current layer, $N$ is the batch
size, $F$ is the number of convolutional filters, and $*$ is the
convolutional operator. For fully connected layers, we use one input
(output) scale variable for each input (output) neuron to group weights
connected to that neuron. For convolutional layers, we use only one
input scale variable for all filters and one output scale variable
for each filter output. We use the {[}width, height, filters, batch{]}
dimension ordering. Local reparameterization \cite{kingma2015variational}
is used to efficiently sample the input, output group scale variables,
and the activations.

